Improving performance in multi-objective decision-making in Bottles environments with soft maximin approaches

Balancing multiple competing and conflicting objectives is an essential task for any artificial intelligence tasked with satisfying human values or preferences. Conflict arises both from misalignment between individuals with competing values, but also between conflicting value systems held by a single human. Starting with principle of loss-aversion, we designed a set of soft maximin function approaches to multi-objective decision-making. Bench-marking these functions in a set of previously-developed environments, we found that one new approach in particular, 'split-function exp-log loss aversion' (SFELLA), learns faster than the state of the art thresholded alignment objective method (Vamplew et al, 2021) on three of four tasks it was tested on, and achieved the same optimal performance after learning. SFELLA also showed relative robustness improvements against changes in objective scale, which may highlight an advantage dealing with distribution shifts in the environment dynamics. Due to publishing rules, further work could not be presented in the preprint, but in the final published version, we will further compare SFELLA to the multi-objective reward exponentials (MORE) approach (Rolf, 2020), demonstrating that SFELLA performs similarly to MORE in a simple previously-described foraging task, but in a modified foraging environment with a new resource that was not depleted as the agent worked, SFELLA collected more of the new resource with very little cost incurred in terms of the old resource. Overall, we found SFELLA useful for avoiding problems that sometimes occur with a thresholded approach, and more reward-responsive than MORE while retaining its conservative, loss-averse incentive structure.

==> granularity_diff_summary.tex <==

\begin{tabular}{>{\raggedright\arraybackslash}p{5em}>{\raggedleft\arraybackslash}p{4em}>{\raggedright\arraybackslash}p{4.5em}rrrrrlrlrrrrrlr}
\toprule
Agent & Environment & R0_P0.01 & R0_P0.1 & R0_P1 & R0_P10 & R0_P100 & R0.01_P0 & R0.01_P0.01 & R0.1_P0 & R0.1_P0.1 & R1_P0 & R1_P1 & R10_P0 & R10_P10 & R100_P0 & R100_P100 & GranularityZero\\
\midrule
 & Breakable Bottles & 1.51 & 1.44 & 1.46 & 1.46 & 1.58 & 1.42 & 1.48 & 1.42 & 1.23** & 1.09** & 0.98*** & -6.46*** & -11.14*** & -41.39*** & -81.28*** & 1.54\\
\cmidrule{2-18}
 & Doors & 1.50 & 1.47 & 1.39 & -1.11*** & -1.08*** & 0.92*** & 0.55*** & 1.23* & 0.31*** & 1.17** & 0.18*** & -7.90*** & -15.34*** & -41.87*** & -63.15*** & 1.42\\
\cmidrule{2-18}
 & Sokoban & -15.01 & -14.98 & -14.96 & -15.03 & -14.99 & -14.99 & -15.01 & -14.91 & -14.98 & -14.86** & -14.92 & -15.04 & -20.38*** & -10.52*** & -51.21*** & -14.97\\
\cmidrule{2-18}
\multirow[t]{-4}{5em}{\raggedright\arraybackslash EEBA1} & Unbreakable Bottles & 28.73 & 28.70 & 28.70 & 28.73 & 28.76 & 28.73 & 28.72 & 28.76 & 28.63* & 28.64* & 28.22*** & 23.22*** & 18.57*** & -13.27*** & -29.84*** & 28.73\\
\cmidrule{1-18}
 & Breakable Bottles & 1.46 & 1.49 & 1.43 & 1.51 & 1.44 & 1.58 & 1.38 & 1.43 & 1.31 & 1.48 & 1.60 & -527.98*** & -531.74*** & -544.06*** & -549.61*** & 1.47\\
\cmidrule{2-18}
 & Doors & -1.07 & -1.18 & -1.04 & -1.06 & -0.86 & -1.18 & -1.03 & -1.19 & -1.08 & -1.12 & -1.13 & -4.21*** & -9.52*** & -4.10*** & -10.07*** & -1.05\\
\cmidrule{2-18}
 & Sokoban & -14.96* & -14.99 & -14.97 & -15.00 & -14.95* & -15.00 & -15.00 & -14.99 & -15.00 & -14.98 & -14.99 & -15.89*** & -15.91*** & -15.93*** & -15.92*** & -15.04\\
\cmidrule{2-18}
\multirow[t]{-4}{5em}{\raggedright\arraybackslash EEBA2} & Unbreakable Bottles & 28.71 & 28.69 & 28.71 & 28.75 & 28.72 & 28.75 & 28.71 & 28.73 & 28.74 & 28.73 & 28.74 & -458.97*** & -124.48*** & -458.83*** & -127.06*** & 28.76\\
\cmidrule{1-18}
 & Breakable Bottles & 4.65 & 5.29*** & 4.83** & 2.28*** & 2.13*** & 4.52 & 4.52 & 4.38 & 5.32*** & 4.32 & 3.88*** & -6.62*** & -12.95*** & -40.36*** & -81.01*** & 4.49\\
\cmidrule{2-18}
 & Doors & -1.85*** & -1.17*** & -0.27*** & -4.98*** & -4.84*** & -9.13 & -1.87*** & -9.68*** & -1.51*** & -11.38*** & -2.73*** & -11.22*** & -16.99*** & -39.14*** & -63.41*** & -9.02\\
\cmidrule{2-18}
 & Sokoban & 5.12*** & 5.02*** & -14.62*** & -20.12*** & -20.19*** & 5.74 & 5.00*** & 5.69 & 4.97*** & 5.50* & -14.32*** & 2.63*** & -23.81*** & -10.03*** & -51.44*** & 5.72\\
\cmidrule{2-18}
\multirow[t]{-4}{5em}{\raggedright\arraybackslash ELA1} & Unbreakable Bottles & 17.91*** & 20.38*** & 21.51*** & 20.94*** & 21.07*** & 16.70 & 17.93*** & 16.65 & 20.45*** & 16.57 & 21.41*** & 10.27*** & 15.96*** & -7.62*** & -29.72*** & 16.55\\
\cmidrule{1-18}
 & Breakable Bottles & -2.29 & -2.21 & -2.21 & -2.10 & -2.23 & -2.25 & -2.15 & -2.25 & -2.34 & -2.23 & -2.24 & -545.16*** & -549.90*** & -543.25*** & -547.82*** & -2.30\\
\cmidrule{2-18}
 & Doors & -0.61 & -0.64 & -0.58 & -0.82 & -0.64 & -0.54 & -0.58 & -0.61 & -0.54 & -0.61 & -0.57 & -4.27*** & -11.28*** & -4.21*** & -9.65*** & -0.70\\
\cmidrule{2-18}
 & Sokoban & -14.95 & -14.93 & -14.93 & -14.89 & -14.91 & -14.95 & -14.90 & -14.91 & -14.87 & -14.93 & -14.93 & -15.95*** & -15.98*** & -15.94*** & -15.96*** & -14.94\\
\cmidrule{2-18}
\multirow[t]{-4}{5em}{\raggedright\arraybackslash ELA2} & Unbreakable Bottles & 28.67 & 28.74 & 28.73 & 28.74 & 28.73 & 28.72 & 28.75 & 28.68 & 28.72 & 28.74 & 28.68 & -459.24*** & -76.19*** & -459.19*** & -96.82*** & 28.74\\
\cmidrule{1-18}
 & Breakable Bottles & 1.83 & 1.81 & 1.73 & 1.76 & 1.70 & 1.75 & 1.85 & 1.67 & 1.79 & 1.75 & 1.86 & -522.84*** & -534.56*** & -542.62*** & -551.04*** & 1.79\\
\cmidrule{2-18}
 & Doors & -0.23** & -0.38 & -0.33 & -0.58 & -0.60 & -0.44 & -0.36 & -0.37 & -0.46 & -0.35 & -0.33 & -4.64*** & -9.12*** & -4.51*** & -10.03*** & -0.47\\
\cmidrule{2-18}
 & Sokoban & -14.86 & -14.88 & -14.86 & -14.87 & -14.87 & -14.89 & -14.89 & -14.91 & -14.90 & -14.87 & -14.89 & -15.95*** & -15.93*** & -15.95*** & -15.93*** & -14.91\\
\cmidrule{2-18}
\multirow[t]{-4}{5em}{\raggedright\arraybackslash LELA2} & Unbreakable Bottles & 28.72 & 28.80 & 28.76 & 28.67* & 28.67* & 28.70 & 28.77 & 28.71 & 28.73 & 28.77 & 28.74 & -459.28*** & -108.78*** & -458.94*** & -79.80*** & 28.78\\
\cmidrule{1-18}
 & Breakable Bottles & 1.47 & 1.40 & 1.57 & 1.35 & 1.44 & 1.38 & 1.46 & 1.48 & 1.47 & 1.46 & 1.43 & 1.45 & 1.52 & 1.49 & 1.38 & 1.54\\
\cmidrule{2-18}
 & Doors & -0.48 & -0.57 & -0.51 & -0.42 & -0.45 & -0.47 & -0.61 & -0.37 & -0.54 & -0.46 & -0.50 & -0.46 & -0.43 & -0.38 & -0.43 & -0.53\\
\cmidrule{2-18}
 & Sokoban & -14.97 & -14.97 & -14.96 & -15.01 & -15.05 & -15.00 & -14.98 & -14.94* & -15.01 & -14.98 & -15.03 & -14.99 & -14.98 & -14.96 & -14.99 & -15.03\\
\cmidrule{2-18}
\multirow[t]{-4}{5em}{\raggedright\arraybackslash LIN_SUM} & Unbreakable Bottles & 28.72 & 28.70 & 28.71 & 28.76 & 28.77 & 28.76 & 28.75 & 28.75 & 28.69* & 28.73 & 28.74 & 28.74 & 28.79 & 28.74 & 28.73 & 28.79\\
\cmidrule{1-18}
 & Breakable Bottles & 4.13 & 4.80*** & 4.41* & 2.46*** & 2.36*** & 4.08 & 4.06 & 3.93* & 4.67*** & 3.80*** & 3.29*** & -6.47*** & -12.93*** & -40.47*** & -81.14*** & 4.16\\
\cmidrule{2-18}
 & Doors & -2.44*** & -1.44*** & -0.82*** & -5.50*** & -5.48*** & -9.61 & -2.33*** & -10.21*** & -2.07*** & -12.18*** & -3.43*** & -11.42*** & -17.04*** & -40.56*** & -63.68*** & -9.64\\
\cmidrule{2-18}
 & Sokoban & 4.56*** & 4.45*** & -14.37*** & -20.53*** & -20.68*** & 4.93 & 4.54*** & 5.23 & 4.47*** & 4.92*** & -16.05*** & 2.83*** & -23.76*** & -10.97*** & -51.31*** & 5.27\\
\cmidrule{2-18}
\multirow[t]{-4}{5em}{\raggedright\arraybackslash ROLF_EXP_LOG1} & Unbreakable Bottles & 17.50*** & 19.72*** & 20.63*** & 20.42*** & 20.31*** & 16.23 & 17.60*** & 16.30 & 19.58*** & 16.07*** & 20.50*** & 9.94*** & 16.12** & -9.15*** & -29.94*** & 16.37\\
\cmidrule{1-18}
 & Breakable Bottles & -10.26 & -10.38 & -9.87 & -9.59 & -18.94*** & -10.36 & -10.15 & -10.19 & -9.84 & -10.19 & -8.94*** & -17.23*** & -24.84*** & -0.03*** & -49.42*** & -10.11\\
\cmidrule{2-18}
 & Doors & -3.04 & -2.94 & -2.90 & -3.75*** & -8.61*** & -2.91 & -3.30* & -2.93 & -2.82 & -2.86 & -3.60*** & -7.66*** & -19.92*** & -0.16*** & -41.01*** & -2.89\\
\cmidrule{2-18}
 & Sokoban & -18.06 & -18.23 & -18.21 & -19.17*** & -22.72*** & -18.19 & -18.18 & -18.32 & -18.35 & -18.37 & -18.85*** & -22.34*** & -28.28*** & -14.42*** & -35.96*** & -18.01\\
\cmidrule{2-18}
\multirow[t]{-4}{5em}{\raggedright\arraybackslash ROLF_EXP_LOG2} & Unbreakable Bottles & 20.18 & 20.27 & 20.16 & 20.02 & 15.60*** & 20.13 & 20.18 & 20.22 & 20.20 & 19.83* & 20.10 & 13.34*** & 9.24*** & 28.16*** & -6.41*** & 20.14\\
\cmidrule{1-18}
 & Breakable Bottles & 1.44 & 1.51 & 1.42 & 1.48 & 1.50 & 1.38 & 1.37 & 1.57 & 1.41 & 0.89*** & 0.99** & -7.65*** & -11.18*** & -19.78*** & -81.11*** & 1.40\\
\cmidrule{2-18}
 & Doors & -0.46 & -0.38 & -0.57 & -0.95*** & -0.86*** & 0.50*** & 0.29*** & 0.43*** & -0.03*** & -0.53 & -1.13*** & -9.48*** & -15.37*** & -41.19*** & -63.70*** & -0.46\\
\cmidrule{2-18}
 & Sokoban & -14.99 & -15.01 & -14.94 & -14.99 & -15.00 & -15.00 & -14.97 & -14.96 & -14.94 & -14.87 & -14.96 & -15.10 & -20.47*** & -9.50*** & -51.12*** & -14.94\\
\cmidrule{2-18}
\multirow[t]{-4}{5em}{\raggedright\arraybackslash SEBA1} & Unbreakable Bottles & 28.72 & 28.73 & 28.76 & 28.75 & 28.76 & 28.74 & 28.71 & 28.68* & 28.60*** & 28.59*** & 28.19*** & 22.71*** & 18.44*** & -1.04*** & -29.92*** & 28.78\\
\cmidrule{1-18}
 & Breakable Bottles & 1.41 & 1.52 & 1.48 & 1.46 & 1.50 & 1.49 & 1.48 & 1.32 & 1.41 & 1.50 & 1.52 & -530.55*** & -528.00*** & -545.18*** & -549.76*** & 1.51\\
\cmidrule{2-18}
 & Doors & -1.73 & -1.55 & -1.53 & -1.11*** & -0.95*** & -1.57 & -1.61 & -1.56 & -1.69 & -1.68 & -1.66 & 1.80*** & -11.24*** & 1.55*** & -10.98*** & -1.68\\
\cmidrule{2-18}
 & Sokoban & -15.00 & -15.02 & -14.98 & -14.95 & -14.96 & -14.99 & -14.97 & -15.02 & -15.00 & -14.98 & -14.99 & -15.91*** & -15.93*** & -15.97*** & -15.89*** & -14.99\\
\cmidrule{2-18}
\multirow[t]{-4}{5em}{\raggedright\arraybackslash SEBA2} & Unbreakable Bottles & 28.64 & 28.62 & 28.61 & 28.68 & 28.77 & 28.64 & 28.60 & 28.63 & 28.61 & 28.60 & 28.68 & -479.39*** & -98.02*** & -476.28*** & -94.66*** & 28.67\\
\cmidrule{1-18}
 & Breakable Bottles & 6.61 & 6.52 & 4.08*** & 1.44*** & 1.39*** & 6.47 & 6.49 & 6.56 & 6.37** & 6.37** & 4.13*** & -5.41*** & -11.25*** & -40.38*** & -81.19*** & 6.61\\
\cmidrule{2-18}
 & Doors & 4.02*** & 4.12*** & 4.64 & -0.94*** & -1.02*** & 3.96*** & 2.84*** & 3.98*** & 3.05*** & 3.80*** & 3.06*** & -10.90*** & -15.31*** & -39.01*** & -63.28*** & 4.62\\
\cmidrule{2-18}
 & Sokoban & -10.31 & -11.44 & -14.90*** & -14.96*** & -15.01*** & -10.83 & -11.61 & -9.67 & -11.56 & -7.43 & -14.80*** & 5.63*** & -20.47*** & -9.44 & -51.48*** & -9.32\\
\cmidrule{2-18}
\multirow[t]{-4}{5em}{\raggedright\arraybackslash SFLLA1} & Unbreakable Bottles & 27.94 & 27.92 & 28.77*** & 28.72*** & 28.72*** & 27.91 & 27.88 & 27.96 & 27.88 & 27.79** & 28.25*** & 22.53*** & 18.41*** & -8.23*** & -29.76*** & 27.95\\
\cmidrule{1-18}
 & Breakable Bottles & -1.84 & -1.82 & -1.84 & -1.71 & -1.56 & -1.63 & -1.86 & -1.66 & -1.79 & -1.85 & -1.88 & -542.49*** & -546.28*** & -544.76*** & -550.13*** & -1.80\\
\cmidrule{2-18}
 & Doors & -0.63 & -0.57 & -0.53 & -0.61 & -0.76 & -0.61 & -0.56 & -0.60 & -0.45 & -0.54 & -0.63 & -4.13*** & -10.19*** & -4.14*** & -10.62*** & -0.64\\
\cmidrule{2-18}
 & Sokoban & -14.94 & -14.92 & -14.89 & -14.88* & -14.92 & -14.87* & -14.91 & -14.92 & -14.91 & -14.92 & -14.89 & -15.93*** & -16.00*** & -15.95*** & -15.92*** & -14.97\\
\cmidrule{2-18}
\multirow[t]{-4}{5em}{\raggedright\arraybackslash SFLLA2} & Unbreakable Bottles & 28.73 & 28.72 & 28.73 & 28.75 & 28.70 & 28.74 & 28.75 & 28.72 & 28.77 & 28.72 & 28.78 & -456.53*** & -102.87*** & -459.13*** & -134.72*** & 28.72\\
\cmidrule{1-18}
 & Breakable Bottles & 1.54 & 1.38 & 1.55 & 1.52 & 1.57 & 1.55 & 1.48 & 1.36 & 1.33 & 1.03** & 1.19 & -6.50*** & -11.20*** & -23.36*** & -80.96*** & 1.40\\
\cmidrule{2-18}
 & Doors & 1.44 & 1.49 & 1.31 & -0.89*** & -0.97*** & 5.15*** & 4.81*** & 5.02*** & 4.94*** & 5.03*** & 3.59*** & -7.50*** & -15.41*** & -38.19*** & -63.89*** & 1.39\\
\cmidrule{2-18}
 & Sokoban & -14.96 & -14.98 & -14.95 & -14.97 & -15.00 & -15.01 & -14.97 & -14.93 & -14.91 & -14.84** & -14.96 & -15.05 & -20.40*** & -9.34*** & -51.23*** & -14.95\\
\cmidrule{2-18}
\multirow[t]{-4}{5em}{\raggedright\arraybackslash SFMLA1} & Unbreakable Bottles & 28.71* & 28.68* & 28.76 & 28.72 & 28.74 & 28.70* & 28.75 & 28.77 & 28.60*** & 28.61*** & 28.24*** & 23.20*** & 18.43*** & 0.80*** & -29.89*** & 28.80\\
\cmidrule{1-18}
 & Breakable Bottles & 1.45 & 1.61 & 1.65 & 1.65 & 1.64 & 1.53 & 1.52 & 1.70 & 1.54 & 1.61 & 1.66 & -523.97*** & -533.97*** & -546.02*** & -548.61*** & 1.67\\
\cmidrule{2-18}
 & Doors & -0.62 & -0.52 & -0.61 & -0.74 & -0.82* & -0.55 & -0.58 & -0.57 & -0.60 & -0.65 & -0.55 & -4.44*** & -10.45*** & -4.50*** & -9.94*** & -0.63\\
\cmidrule{2-18}
 & Sokoban & -14.87 & -14.91 & -14.92 & -14.94 & -14.93 & -14.87 & -14.95 & -14.94 & -14.92 & -14.90 & -14.87 & -15.91*** & -15.89*** & -15.94*** & -16.01*** & -14.92\\
\cmidrule{2-18}
\multirow[t]{-4}{5em}{\raggedright\arraybackslash SFMLA2} & Unbreakable Bottles & 28.77 & 28.73 & 28.82 & 28.69 & 28.73 & 28.73 & 28.73 & 28.76 & 28.76 & 28.72 & 28.79 & -460.72*** & -87.58*** & -458.57*** & -87.88*** & 28.73\\
\bottomrule
\end{tabular}

